Machine Learning LSST 3x2pt analyses -- forecasting the impact of systematics on cosmological constraints using neural networks

Validating modeling choices through simulated analyses and quantifying the impact of different systematic effects will form a major computational bottleneck in the preparation for 3$\times$2 analysis with Stage-IV surveys such as Vera Rubin Observatory's Legacy Survey of Space and Time (LSST). We can significantly reduce the computational requirements by using machine learning based emulators, which allow us to run fast inference while maintaining the full realism of the data analysis pipeline. In this paper, we use such an emulator to run simulated 3$\times$2 (cosmic shear, galaxy-galaxy lensing, and galaxy clustering) analyses for mock LSST-Y1/Y3/Y6/Y10 surveys and study the impact of various systematic effects (galaxy bias, intrinsic alignment, baryonic physics, shear calibration and photo-$z$ uncertainties). Closely following the DESC Science Requirement Document (with several updates) our main findings are: {\it a)} The largest contribution to the `systematic error budget' of LSST 3$\times$2 analysis comes from galaxy bias uncertainties, while the contribution of baryonic and shear calibration uncertainties are significantly less important. {\it b)} Tighter constraints on intrinsic alignment and photo-$z$ parameters can improve cosmological constraints noticeably, which illustrates synergies of LSST and spectroscopic surveys. {\it c)} The scale cuts adopted in the DESC SRD may be too conservative and pushing to smaller scales can increase cosmological information significantly. {\it d)} We investigate the impact of photo-$z$ outliers on 3$\times$2 pt analysis and find that we need to determine the outlier fraction to within $5-10\%$ accuracy to ensure robust cosmological analysis. We caution that these findings depend on analysis choices (parameterizations, priors, scale cuts) and can change for different settings.

==> sections_deprecated/background.tex <==
% \newpage

\section{Theoretical Basics}\label{sec:background}

\subsection{Theoretical modeling of the data vectors}\label{ssec:model_data_vector}

Our 3x2 data vector is comprised of real-space two point correlation functions which requires the calculation of projected angular power spectra for the convergence field and galaxy density field. The angular power spectrum of two observables, $A$ and $B$ (here, $A/B$ stand for either the convergence field or the galaxy density field) for a Fourier mode, $\ell$ is given in terms of the 3D power spectrum $P_{AB}$ as,

\begin{equation}\label{eqn:angular_power_spectra}
    C^{ij}_{AB}(\ell) = \int_0^{\chi_{\text{H}}} d\chi \frac{q^{i}_A(\chi) q^{j}_B(\chi)}{\chi^2} P_{AB}\bigg[ \frac{\ell + 1/2}{\chi}, z(\chi) \bigg],
\end{equation}
where, the Latin indices ($i/j$) label the tomographic bin. The weight kernels $q$ for the galaxy density field, $\delta_g$ and the convergence field, $\kappa$ are given as,
\begin{align}
    q^i_{\delta_g}(\chi) &= \frac{n^i[z(\chi)]}{\bar{n}^i} \frac{\diffop z}{\diffop \chi},\\
    q_{\kappa}(\chi) &= \frac{3 H^2_0 \Omega_m}{2c^2} \frac{\chi}{a(\chi)} \int_{\chi}^{\chi_{\text{H}}} \diffop \chi^{\prime} \frac{\diffop z}{\diffop \chi^{\prime}} \frac{n^i[z(\chi^{\prime})]}{\bar{n}^i} \frac{\chi^{\prime} - \chi}{\chi^{\prime}}.
\end{align}
In the above, $n^i(z)$ denotes the redshift distribution of galaxies in the $i$-the tomographic bin, $\chi$ denotes the comoving distance, $\chi_{\text{H}}$ denotes the comoving horizon distance, $a$ is the scale factor, $\bar{n}^i$ is the mean number density of source/lens galaxies. 

In case of the lens sample being different from the source sample, the $n(z)$ entering both equations are different, however we use the source sample itself as a lens sample; therefore we use the same $n(z)$ in both kernels. The power spectrum entering equation \eqref{eqn:angular_power_spectra} is related to the non-linear matter power spectrum, $P_{\delta\delta}$, which we calculate assuming the {\sc halofit} prescription \citep{Takahashi2012}. The power spectra associated with the galaxy density field and the convergence field are given as,
\begin{align}
    P_{\delta_g B}(k,z) &= b_g(z) P_{\delta B}(k, z), \\
    P_{\kappa B}(k, z) &= P_{\delta B}(k, z),
\end{align}
where, $B$ stands for $\delta_g/\kappa$. In the above, we have also assumed the Limber approximation \citep{Limber1953, LoVerde2008}. 

The real space correlation functions are given in terms of the angular power spectra as \citep{Krause2021}, 
\begin{align}    
    \xi^{ij}_{\pm} &= \sum_{\ell} \frac{2\ell + 1}{2\pi \ell^2 (\ell + 1)^2}[G^{+}_{\ell,2}(\cos \theta) \pm G^{-}_{\ell,2}(\cos \theta)] C_{\kappa\kappa}^{ij}(\ell), \label{eqn:xi_cosmic_shear}\\
    \gamma^{ij}_t(\theta) &= \sum_{\ell} \frac{(2\ell + 1)}{2\pi \ell^2 (\ell + 1)^2} P^2_{\ell}(\cos \theta) C^{ij}_{\delta_g \kappa}, \label{eqn:gammat_ggl}\\
    w^{i}(\theta) &= \sum_{\ell} \frac{2\ell + 1}{4\pi} P_{\ell}(\cos \theta) C^{ii}_{\delta_g \delta_g} (\ell). \label{eqn:w_clustering}
\end{align}
In the above, $P_{\ell}$ and $P^2_{\ell}$ are the Legendre and associated Legendre polynomials. The functions $G^{\pm}_{\ell,2}$ are given in \citep{Stebbins1996}. Finally, to compare against the measurement of the correlation function, we average the correlation functions in angular bins. The details of the scale cuts and angular bins used in this work is given in section \ref{ssec:scale_cuts}. 

%Since we study 3$\times$2 point analysis in this paper, the data vector, $\mvec{d}$, is a concatenated data vector consisting of the cosmic shear, galaxy-galaxy lensing and the galaxy clustering data vectors. 
% In this work, we perform a real space analysis that uses the two-point correlation function as the data vector. 





We use {\sc cocoa} to compute the model data vectors on which our emulator is trained (section \ref{ssec:emulator}). While sampling, we use the trained emulator to predict the model data vector, thus resulting in fast inference. 


\subsection{Simulated likelihood analysis}\label{ssec:simulated_analyses}

To gauge the impact of systematic effects on cosmological constraining power we conduct simulated likelihood analyses in a joint parameter space of cosmological parameters and systematics parameters.

We compute the posterior probability in parameter space as 
\begin{equation}\label{eqn:bayes}
    \mP(\mtheta|\md_{\text{sim}}) \propto \mL(\mtheta|\md_{\text{sim}}) \mP(\mtheta),
\end{equation}
where, $\mtheta$ is the collection of cosmological and systematic parameters and $\mP(\mtheta)$ is the prior on these parameters. In the above equation, $\mL$ is the likelihood function which is assumed to be Gaussian
\begin{equation}\label{eqn:log_lkl}
    \log \mL(\mtheta|\md_{\text{sim}}) = -\frac{1}{2} 
    [\md_{\text{model}}(\mtheta) - \md_{\text{sim}}]^{\text{T}} \mmat{C}^{-1} [\md_{\text{model}}(\mtheta) - \md_{\text{sim}}].
\end{equation}
 
The data vectors $\md_{\text{sim}}$ are computed at a fiducial point in parameter space (see Table \ref{tbl:parameters}), the model vectors $\mvec{d}_{\text{model}}$ are computed as a function of cosmological and systematic parameters, and $\mmat{C}$ is the covariance of the data vector.

We use the {\sc cocoa}\footnote{\url{https://github.com/CosmoLike/Cocoa}} framework \citep{Miranda:2020lpk} to compute the data and  model vectors following the prescription of the previous section. {\sc cocoa}({\sc cobaya}-{\sc cosmolike} {\sc architecture}) integrates \cosmolike \citep{Krause2017},  into the {\sc cobaya} likelihood framework \citep{Torrado2021}.


We use {\sc cosmocov} \citep{Fang2020} to calculate the covariance for our 3$\times$2 point analyses. {\sc cosmocov}\footnote{\url{https://github.com/CosmoLike/CosmoCov}} is a publicly available code that uses analytical calculations to compute the covariance of the real-space correlation functions including the super-sample and the connected non-Gaussian part of the covariance. The code has been used to compute the 3x2 real space covariances for the relevant DES analyses \citep{DESY1, DES_3x2} and the Fourier covariance for the DESC-SRD \citep{DESC_SRD}. We refer the reader to \citet{Krause2017, Fang2020, Krause2021} for exact details of the covariance calculation.


The calculation of the model vector during the MCMC is a significant computational cost. In this paper, the model vector is computed with the help of an emulator that speeds up the calculation by orders of magnitude (see section \ref{ssec:emulator}).


% In this paper, we compute the covariances for the different mock surveys including all the components, namely, the Gaussian, super sample covariance and the connected non-Gaussian part of the covariance. 
% \cyan{The Gaussian part of the covariance also contains the shape (shot) noise for the source (lens) galaxies. We do not consider any spatial variation of these noise in the covariance. 


%=====================================================
\subsection{Neural Network Emulator}\label{ssec:emulator}
%=====================================================

In this paper we train the same 3 layer, fully connected neural network architecture (1024 neurons, ReLU activation function) as in \cite{Boruah2022} to predict the model data vector as a function of the cosmological and systematic parameters. We add one minor modification in that we train $4$ different neural networks to separately predict the $\xi_{+}$, $\xi_{-}$, $\gamma_t$ and $w$ parts of the model vector, instead of training one network for all parts. 

Even with extensive training, a brute force approach of building an emulator over the full prior range of the high-dimensional parameter space of LSST 3$\times$2 analyses did not yield sufficiently accurate results. Similar to \cite{Boruah2022} we solve this problem by combining two ideas: Firstly, we shrink the emulated parameter space by separating ``slow'' and ``fast'' parameters ({\cyan also see LEWIS for this idea)}. The former are included in the emulator and the latter are applied after the emulator has returned its result. Examples for slow parameters are cosmological parameter, IA, and photo-z parameters, examples for fast parameters in our implementation are baryonic uncertainties, galaxy bias, and shear calibration. Secondly, we implement an iterative design, where we acquire training samples from a tempered posterior that is obtained from an MCMC analysis using the emulator from the previous iteration. In that way, we acquire more training samples in the high posterior region, which is significantly smaller than the full prior range. The combination of these ideas gives excellent results for an LSST likelihood analysis after 3-4 iterations of training the neural network \citep[see][for details]{Boruah2022}. 

We note that this type of iterative local training reduces the walltime of an MCMC signficantly since the calculation of the training sample can be fully parallelized during each iteration. Since the subsequent emulator based MCMC only takes minutes, the main computational bottleneck is the training of the neural network. Including emlator training, the walltime of such an MCMC is of order 1h; all subsequent chains using this trained emulator run within minutes, using one chain per core. 

We note the limitations of our locally trained emulators, especially in the context of impact studies (see sections \ref{sec:photoz_outliers}, \ref{ssec:impact_studies}), where the data vector is computed several $\sigma$ away from the central parameter point around which the emulator was trained. {\cyan Need statement about approximate accuracy of the emu}. Since our emulator is sufficiently accurate for the results presented in this paper we refrain from exploring alternative neural network architectures. We note that accurately predicting the model vector over a larger parameter space, perhaps even the full LSST 3x2 prior range are an important and active research area. 

% Furthermore, the emulator utilizes the fact that some of the parameters, such as the linear galaxy bias and the shear multiplicative bias affects the data vector in a simple way. These parameters are not included in the emulated parameters and their effects are added simply at the end. Following these designs, we get an emulator that can speed up 3$\times$2 point analysis by two orders of magnitude. Therefore, using this emulator, we can perform extremely fast analysis while preserving the realism in the aspects of modeling. 

%For brevity, we refer to \citet{Boruah2022} for further details on the design of the emulator. 



==> sections_deprecated/error_budget.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/error_budget/systematic_error_budget_1sys.pdf}
%     \caption{Dark energy figure of merit calculated for MCMC chains run by fixing one set of systematic parameters to their fiducial values. The FoM for the chain where all the systematic parameters are marginalized is shown with a solid dark blue bar. As can be seen, marginalization of the galaxy bias  has the largest impact on the dark energy figure-of-merit. On the other hand, marginalization over baryonic effects have a negligible impact on the DE FoM. See section \ref{ssec:error_budget} for more details.}
%     \label{fig:systematics_error_budget}
% \end{figure}

% \iffalse
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/error_budget/fom_combinations.pdf}
    \caption{$w_0$-$w_a$ Figure-of-merit budget for all combinations of systematics. The different hatches in the legend shows systematic parameter that is varied in a given chain. For example, when the red dotted hatch is present, the photo-$z$ bias parameters are varied. The size of the different bars are equal and \textit{do not} denote the contribution of different systematics. When multiple systematic parameter combinations are varied, it captures the contribution from the correlated systematic parameters in the chain.}
    \label{fig:fom_combinations}
\end{figure*}

\begin{table*}
  \centering
  \caption{The dark energy figure-of-merit for different combination of systematic parameters. }
  \begin{tabular}{l c c c c}
  \hline
     Varied systematic parameters &  LSST-Y1 & LSST-Y3 & LSST-Y6 & LSST-Y10\\
    \hline
    \textbf{None (Cosmo only)} & 54 & 121 & 172 & 224 \\
    \hline
    \textbf{Vary 1 set of systematic parameters} & & & & \\
    Photo-$z$ & 45 & 95 & 140 & 190 \\    
    IA & 42 & 97 & 141 & 187 \\    
    Galaxy bias & 30 & 76 & 102 & 125 \\    
    Shear calibration & 46 & 114 & 159 & 203 \\    
    Baryons & 53 & 117 & 170 & 226 \\    
    \hline
    \textbf{Vary 2 sets of systematic parameters} & & & & \\
    Photo-$z$, IA & 34 & 75 & 112 & 154 \\  
    Photo-$z$, Galaxy bias & 29 & 63 & 78 & 89 \\  
    Photo-$z$, Shear calibration & 41 & 86 & 132 & 184\\  
    Photo-$z$, Baryons & 45 & 94 & 139 & 191 \\  
	IA, Galaxy bias & 22 & 60 & 80 & 98  \\  
    IA, Shear calibration & 36 & 88 & 124 & 160  \\  
    IA, Baryons & 42 & 96 & 142 & 193 \\  
    Galaxy bias, Shear calibration & 27 & 67 & 85 & 99\\  
    Galaxy bias, Baryons & 30 & 74 & 92 & 105 \\  
    Shear calibration, Baryons & 46 & 107 & 160 & 218 \\  
    \hline
    \textbf{Vary 3 sets of systematic parameters} & & & & \\
    Galaxy bias, Shear calibration, Baryons & 30 & 65 & 88 & 109 \\  
    IA, Shear calibration, Baryons & 42 & 87 & 145 & 219 \\  
    IA, Galaxy bias, Baryons & 25 & 55 & 74 & 93 \\  
    IA, Galaxy bias, Shear calibration, & 20 & 54 & 70 & 78 \\  
	Photo-$z$, Shear calibration, Baryons & 44 & 86 & 131 & 186\\  
    Photo-$z$, Galaxy bias, Baryons & 29 & 59 & 73 & 80 \\  
    Photo-$z$, Galaxy bias, Shear calibration & 28 & 58 & 74 & 88 \\  
    Photo-$z$, IA, Baryons & 36 & 71 & 112 & 162 \\  
    Photo-$z$, IA, Shear calibration & 31 & 67 & 101 & 138 \\  
    Photo-$z$, IA, Galaxy bias & 22 & 45 & 58 & 67 \\  
    \hline
    \textbf{Vary 4 sets of systematic parameters} & & & & \\    
	IA, Galaxy bias, Shear calibration, Baryons [Photo-$z$ fixed] & 24 & 50 & 66 & 81 \\  
    Photo-$z$, Galaxy bias, Shear calibration, Baryons [IA fixed] & 28 & 54 & 72 & 90 \\  
    Photo-$z$, IA, Shear calibration, Baryons [Galaxy bias fixed] & 35  & 66 & 104 & 152 \\  
    Photo-$z$, IA, Galaxy bias, Baryons [Shear calibration fixed] & 21 & 44 & 54 & 61 \\  
	Photo-$z$, IA, Galaxy bias, Shear calibration [Baryons fixed] & 20 & 41 & 51 & 56 \\  
    \hline
    \textbf{Vary all systematics} & 20 & 38 & 51 & 66 \\  
    \hline
  \end{tabular}
  \label{tbl:sys_error_budget}
\end{table*}
% \fi 

\section{Mapping impact of systematics}\label{sec:science_return_map}

% At the precision levels of LSST, the systematic errors will become more important and will likely dominate over the statistical error. For the purposes of constraining cosmological parameters, it is desirable that the systematic uncertainties contribute as small a fraction of the overall error budget \citep{DESC_SRD}. 
% There are different strategies one can use for improved modeling of different systematic effects, which in turn will have the additional benefit of improving the cosmological constraints. This can be achieved through different means. For example, there have been proposals for follow-up spectroscopy in the LSST footprint \citep{Astro2020_spectroscopy1, Astro2020_spectroscopy2, Snowmass} that can improve the constraints on intrinsic alignment and photo-$z$'s. Alternately, one can try to model the various astrophysical systematics using external probes or utilizing numerical simulations. For example, for better modeling of baryons, one can perform joint analysis with thermal Sunyaev-Zeldovich (tSZ) effect \citep{Gatti2022, Pandey2022, Troster2022} or can utilize hydrodynamical simulations to model the effect of baryonic feedback on small-scale power spectrum \citep{Eifler2015, Huang2019}. However, all of these avenues will likely require a lot of resources (either in telescope time or people effort). Hence, identifying the most promising avenues to improve the cosmological constraints will be useful in prioritizing these different efforts. In this section, we use our emulator-based analyses to perform precise forecasting and map out the science returns of constraining different systematic effects. In section \ref{ssec:error_budget}, we quantify the error budget of different systematic effects including the impact of correlated uncertainties. 
% Then in section \ref{ssec:priors}, we run simulated analyses to map out the cosmological gains from putting better constraints on systematics. 
% In reality, however, we will not be able to determine the systematics exactly. Instead, with better observations or modeling, we will be able to put stronger constraints on the different systematic effects. Therefore, we look at the impact of more realistic improvement or degradation in the modeling of different systematic effects in section \ref{ssec:priors} by imposing optimistic and pessimistic priors on different systematic parameters. 


In this paper we pursue two different avenues to quantify the impact of systematics: Firstly, we consider the increase in error budget when marginalizing over nuisance parameters associated with the different types of systematics. Secondly, we study parameter biases that occur when not (properly) accounting for systematics in the analyses. We note that both approaches are affected by the exact parameterization that is assumed for the systematics and results will change as a function of said parameterization and also as a function of other analysis choices, in particular scale cuts (see section \ref{sec:small_scales}) and priors (see section \ref{ssec:priors}).  
\subsection{Systematics error budget}\label{ssec:error_budget}

\iffalse
=============================

To-do:
\begin{itemize}
    \item \red{Differences from DESC-SRD:}
    \begin{enumerate}
        \item \red{The Figure-of-merit is different (lower than) from SRD}
        \item \red{Definition of systematic uncertainty is different from DESC-SRD}
    \end{enumerate}
\end{itemize}
=============================
\fi

% In order to do so, we run MCMC chains by fixing the values of the different systematic parameters to their fiducial values. 
As described in section \ref{ssec:systematics}, we marginalize over 5 different groups of systematic effects, namely, photo-$z$ bias, intrinsic alignment, galaxy bias, shear multiplicative bias, and baryonic modeling uncertainties. We quantify the contribution of each of these systematic sets to the overall error budget individually and in combination. 

In Figure \ref{fig:fom_combinations} we show 128 simulated 3x2 MCMC analyses and quantify the science return with the standard dark energy figure-of-merit (see Table \ref{tbl:sys_error_budget} for the exact numerical values). Each row corresponds to a different LSST dataset (from top to bottom: Y1, Y3, Y6, Y10). We increase the complexity of the analysis (aka the size of the parameter space) from left to right, starting with the cosmology-only analysis and ending with the full likelihood analysis that contains all 5 groups of systematic effects.


Comparing the cosmology-only analysis on the far left to the next set, where we marginalize over each group of the systematics individually, we clearly see that the largest degradation in constraining power comes from the inclusion of galaxy bias uncertainties (green). We further find that intrinsic alignment (yellow) and photo- z uncertainties (red) also cause significant loss in constraining power, with multiplicative shear calibration (blue) being less important, and baryonic uncertainties (dark gray) barely degrading the information content. 


When looking at the column in Figure \ref{fig:fom_combinations} where we look at 4 sets of systematics in combination (last but one), we also see that galaxy bias uncertainties (green) cause the most severe degradation. The FoM for LSST-Y1 (Y10) with fixed galaxy bias is 35 (122) as opposed to 21 (57) when all systematics are marginalized \cyan{not consistent with table}. Thus, marginalization over galaxy bias degrades the DE FoM by a factor of $\sim 1.75$-$2$. On the other hand, marginalizing over baryonic physics has negligible impact on the dark energy figure of merit. For each of LSST-Y1/3/6/10, baryons contribute $\lesssim 5\%$ of the overall error budget to the dark energy figure-of-merit. Similarly, the shear multiplicative bias contributes $\mathcal{O}(10$-$20\%)$ to the overall error budget. Finally, the photo-$z$ bias and intrinsic alignment contribute a significant amount to the overall budget (although not at the level of the galaxy bias). IA contributes $\mathcal{O}(30$-$40\%)$ to the overall error budget for each of the LSST years considered. Marginalization over the photo-$z$ bias contributes a similar amount for LSST-Y10 $\sim \mathcal{O}(40\%)$, for LSST-Y1, the contribution is only $ \sim \mathcal{O}(10\%)$. 

Our analysis above provides a ranking of how much the dark energy equation of state parameters can be improved by finding a better parameterization or better priors for the different systematics groups. However, it is important to note that this ranking will likely look different for other cosmological parameters of interest, e.g. $S_8$ or $H_0$. Further, this ranking can also look different if a different parameter space is considered, e.g. more complex dark energy or modified gravity models, or when different scale cuts are employed. Each parameter space is unique and we stress that a study as the one conducted in Figure \ref{fig:fom_combinations} should be performed early on when defining the analysis choices for a given science case. Our neural network emulator allows for such studies at scale. 

The ranking expressed by Figure \ref{fig:fom_combinations} and Table \ref{tbl:sys_error_budget} will also change if the parameterization of the groups of systematics changes. For example, a parameterization of baryonic physics uncertainties that has more degrees of freedom will impact the cosmological parameter space differently and can also cause a stronger degradation for dark energy parameters. Vice versa, a more confined parameterization of galaxy bias can reduce the degradation we see above. 

For the exact analysis choices of this paper as described in Section \ref{sec:background} we find that LSST 3$\times$2 point analysis are systematics limitedin the sense that systematic effects will contribute more to the overall error budget than statistical uncertainties. Comparing the cosmology-only FoMs in Table \ref{tbl:sys_error_budget} with the FoM where all systematic parameters are varied, we find a factor 2-3 difference depending on the dataset. 




% To do so, we run MCMC chains with certain systematic parameters fixed to their fiducial values. In these runs, we re-use an emulator that has been trained on the full parameter space.  


% Since the contours obtained by fixing certain parameters are always within the contours where all the parameters are marginalized, the emulator is used to predict the data vectors within its training range. We run a number of MCMC chains - first, where all the systematic parameters are marginalized, progressively fixing more and more parameters until we only sample the cosmological parameters. For each of these chains, we calculate the dark energy Figure-of-merit (FoM). This allows us to see which systematic effect contribute the most to the overall error budget. In total this involves running 128 runs (32 for each LSST year) -- something that is nearly unfeasible without the use of the emulator.

% It is useful to first isolate the impact of each systematic effect individually. To do so, we run MCMC chains where each of the 5 sets of systematic parameters are fixed to their fiducial value and compare the results to the chain where all the systematic effects are varied. This is shown in Figure \ref{fig:systematics_error_budget} where we compare the DE FoM for each of these chains to the run with all systematics marginalized. Doing so, we can see which of the systematic effects contribute the most to the overall error budget. As we see from Figure \ref{fig:systematics_error_budget}, fixing galaxy bias to its fiducial values has the largest impact on the dark energy figure of merit. The FoM for LSST-Y1 (Y10) when fixing galaxy bias to its fiducial value is 35 (122) as opposed to 21 (57) when all the systematics are marginalized. Thus, marginalization over galaxy bias degrades the DE FoM by a factor of $\sim 1.75$-$2$. On the other hand, marginalizing over baryonic physics has negligible impact on the dark energy figure of merit. For each of LSST-Y1/3/6/10, baryons contribute $\lesssim 5\%$ of the overall error budget to the dark energy figure-of-merit. Similarly, the shear multiplicative bias contributes $\mathcal{O}(10$-$20\%)$ to the overall error budget. Finally, the photo-$z$ bias and intrinsic alignment contributes a significant amount to the overall budget (although not at the level of the galaxy bias). IA contributes $\mathcal{O}(30$-$40\%)$ to the overall error budget for each of the LSST years considered. Marginalization over the photo-$z$ bias contributes a similar amount for LSST-Y10 $\sim \mathcal{O}(40\%)$. However, for LSST-Y1, the contribution of $\Delta_z$ to the error budget is only $ \sim \mathcal{O}(10\%)$. 

% \iffalse
% Whereas fixing one systematic effect to the truth is illustrative, one might wonder what the impact of correlated uncertainties may be on the cosmological constraints. That is, whether the impact of a small subset of systematic effects capture the bulk of the error budget. The results of this analysis is shown in Figure \ref{fig:fom_combinations}, where we plot the dark energy FoM by fixing different sets of systematic parameters. In Table \ref{tbl:sys_error_budget} we give the numerical results for the dark energy FoM. We note some of the important results of this analysis below:
% \begin{itemize}
%     \item LSST 3$\times$2 point analysis will be systematics limited, meaning that systematic effects will contribute most to the overall error budget. This can be seen by comparing the DE FoM obtained by fixing all the systematic parameters to its fiducial value (top row of Table \ref{tbl:sys_error_budget}) to the FoM when all the systematic parameters are varied (bottom row of Table \ref{tbl:sys_error_budget}). The cosmology only FoM can be larger than the FoM when all the systematic parameters are varied by a factor of $\sim 3$. 
%     \item We saw in Figure \ref{fig:systematics_error_budget} that among the various systematic effects, galaxy bias contributes most to the systematic error budget, followed by intrinsic alignment and photo-$z$ bias. By running the chains with different subsets of systematic parameters fixed, we see that for LSST-Y1, contribution from galaxy bias and intrinsic alignment captures most of the systematic error budget. Just varying these two sets of systematic parameters, while fixing baryons, photo-$z$ and shear calibration bias to its fiducial values gives a FoM that is within $10\%$ of the FoM when all the systematic parameters are marginalized. For later years, the importance of the other contribution increases. However, the contribution of shear calibration bias and baryonic effects to the FoM error budget is always small. Marginalization over these sets of systematic parameters only degrades the DE FoM by a factor of $\sim 10$-$20\%$. 
% \end{itemize}
% % \fi

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/error_budget/priors_plot.pdf}
    \caption{Dark energy Figure of merits for different combinations of optimistic and pessimistic priors. The blue (red) bars correspond to optimistic (pessimistic) prior on $\Delta_z$. The optimistic and pessimistic priors on the intrinsic alignment are denoted with a left slanted ($\ $) and a dense right slanted line hatch ($/$) hatch respectively. The pessimistic priors on shear calibration bias is denoted with dots and the optimistic prior is left unfilled. The corresponding values are given in Table \ref{tbl:priors}.}
    \label{fig:priors_plot}
\end{figure*}

\subsection{Information gain from improved priors}\label{ssec:priors}

\begin{table}
  \centering
  \caption{Optimistic and pessimistic priors used in section \ref{ssec:priors}}
  \begin{tabular}{l c c c}
  \hline
     Systematic &  Pessimistic prior & Optimistic prior\\
    \hline
    \textbf{IA} &  & \\
    $a_1$ & Flat[-5,5]& Gauss[$0.5$, $0.019^2$] for LSST-Y1\\
		 &  & Gauss[$0.5$, $0.015^2$] for LSST-Y3\\
		 &  & Gauss[$0.5$, $0.013^2$] for LSST-Y6\\
		 &  & Gauss[$0.5$, $0.012^2$] for LSST-Y10\\
    $\eta_1$ & Flat[-5,5]& Gauss[$0$, $0.145^2$] for LSST-Y1\\
	& & Gauss[$0$, $0.110^2$] for LSST-Y3\\
	& & Gauss[$0$, $0.091^2$] for LSST-Y6\\
	& & Gauss[$0$, $0.079^2$] for LSST-Y10\\
    \hline 
    \textbf{Photo-$z$ bias} & & \\
    $\Delta_z$ & Gauss(0,$0.005^2$) & Gauss(0,$0.002^2$) for LSST-Y1\\    
    & & Gauss(0,$0.0015^2$) for LSST-Y3\\  
    & & Gauss(0,$0.0015^2$) for LSST-Y6\\  
    & & Gauss(0,$0.001^2$) for LSST-Y10\\  
    \hline   
    \textbf{Shear bias} & & \\
   $m$ & Gauss(0,$0.01^2$) & Gauss(0,$0.005^2$) \\
    \hline 
  \end{tabular}
  \label{tbl:priors}
\end{table}

% \begin{table*}
\begin{table}
  \centering
  \caption{Dark energy figure-of-merit for different combinations of optimistic and pessimistic priors defined in Table \ref{tbl:priors}. The results are shown in Figure \ref{fig:priors_plot}.}
	\begin{tabular}{l|c|c|c c c c}
\hline
% $\Delta_z$ prior & IA prior & $m$ prior & LSST-Y1 & LSST-Y3 & LSST-Y6 & LSST-Y10\\
$\Delta_z$ prior & IA prior & $m$ prior & Y1 & Y3 & Y6 & Y10\\
\hline
\multirow{4}{*}{Pessimistic} & \multirow{2}{*}{Pessimistic} & Pessimistic & 16 & 29 & 35 & 44 \\\cline{3-7}
& & Optimistic & 17 & 30  & 36  & 46 \\\cline{2-7}
    & \multirow{2}{*}{Optimistic} & Pessimistic & 22 & 39 & 48 & 62  \\\cline{3-7}
  & & Optimistic & 22 & 40 & 50 & 66 \\\hline
\multirow{4}{*}{Optimistic} & \multirow{2}{*}{Pessimistic} & 
Pessimistic & 20 & 39 & 50 & 70 \\\cline{3-7}
    & & Optimistic & 21  & 42  & 54  & 74 \\\cline{2-7}
    & \multirow{2}{*}{Optimistic} & Pessimistic & 24 & 47 & 62 & 82 \\\cline{3-7}
    &  & Optimistic & 26 & 50  & 67 & 94  \\\hline
\end{tabular}
\label{tbl:sys_priors}
% \end{table*}
\end{table}

The systematics error budget gave us a way to understand the relative contribution of different systematic effects on the overall error budget. In reality, we cannot infer the value of any parameter exactly. Instead, we may be able to better constrain these parameters with external observations or algorithmic development. For example, there have been proposals for future spectroscopic surveys in the LSST footprint \citep{Astro2020_spectroscopy1, Astro2020_spectroscopy2, Snowmass, megamapper}. These surveys can improve constraints intrinsic alignment parameters and photo-$z$ biases. Similarly, algorithmic developments may achieve stronger constraints on photo-$z$ biases and shear calibration biases. While predicting the exact improvement through these avenues is hard to predict, we simulate different scenarios at a high-level by imposing optimistic and pessimistic priors on different systematic parameters. We perform multiple simulated analyses by considering all combinations of optimistic and pessimistic priors. We briefly describe the choice of our optimistic and pessimistic priors below for different systematics. The different optimistic and pessimistic priors are given in Table \ref{tbl:priors}. 

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/error_budget/opt_pess_ia.png}
    \caption{Optimistic and pessimistic IA results.}
    \label{fig:ia_opt_pess}
\end{figure}
\fi

\begin{itemize}
    \item \textbf{Intrinsic alignment}: In the fiducial case, we assume an uninformative flat prior on the NLA parameters, where the IA parameters are self-calibrated through its impact on the 3$\times$2 point analysis data vector. We consider this the pessimistic scenario for the constraints on the intrinsic alignment parameters. Intrinsic alignment can also be directly constrained using spectroscopic observations \citep{Singh2015, Johnston2019, Samuroff2022, Astro2020_spectroscopy1, Snowmass}. 
    % In the future, intrinsic alignment of LSST galaxies can potentially be constrained using follow-up spectroscopy \citep{Astro2020_spectroscopy1, Snowmass} of LSST galaxies. 
    \citet{Astro2020_spectroscopy1} demonstrated that proposed wide-field spectroscopy of LSST galaxies can yield a 2$\times$ improvement in the signal-to-noise of the IA measurements. Therefore, for the optimistic scenario, we assume that we can put 2$\times$ stronger constraints on the IA parameters with follow-up wide-field spectroscopy. Note that the signal-to-noise does not translate simply to parameter constraints and the 2$\times$ stronger prior on IA parameters is just a simple scheme to approximate an informative prior on IA parameters. For this scenario, we run simulated analyses by using Gaussian priors on the NLA parameters, $a_1$ and $\eta_1$ centred on their fiducial values ($a_1 = 0.5$, $\eta_1 = 0.$) and a standard deviation that is half the value of the standard deviation calculated from the chains run with uninformative prior. 
    
    \item \textbf{Photo-$z$ bias}: In the future, the photo-$z$ characterization can be improved using better spectroscopic samples \citep{Astro2020_spectroscopy1, Astro2020_spectroscopy2} or with algorithmic developments \citep{Sanchez2019,Wright2020,Alsing2023,Leistedt2023}. To check the impact of the accuracy of photo-$z$ characterization on cosmological constraints, we run chains with an optimistic and a pessimistic prior on the photo-$z$ bias. For the optimistic scenario, we assume that the photo-$z$ biases can be constrained
    at the level of LSST requirements \citep{DESC_SRD}, $\sigma[\Delta_z] = 0.002 (0.001)$ for LSST-Y1 (Y10). The optimistic prior for the LSST-Y3/Y6 is taken to be, $\sigma[\Delta_z] = 0.0015$, an intermediate values between the LSST-Y1 and Y10 optimistic values. However, such precise characterization of photo-$z$'s can be challenging to achieve \citep{Newman2022}.    
    Therefore, as our pessimistic scenario, we assume that the photo-$z$'s can be characterized with a standard deviation of $\sigma[\Delta_z] = 0.005$.
    
    \item \textbf{Shear multiplicative bias}: We follow the DESC-SRD to assume a shear multiplicative bias of $\sigma_m = 0.005$ in the optimistic case. As a pessimistic scenario, we assume a standard deviation of $\sigma_m = 0.01$.
    \item \textbf{Baryons}: In the previous section, we saw that marginalizing over baryonic physics have a negligible impact on the cosmological constraints. Therefore, we do not consider any additional scenario for the baryon constraints. Although, we do note that combined analysis with other probes such as thermal Sunyaev-Zeldovich (tSZ) effect can be used to better infer the baryonic physics that impacts the small-scale power spectrum.     
    \item \textbf{Galaxy bias}: It is difficult to obtain stronger constraints on galaxy bias using external probes or new observations. Therefore, we do not consider any additional scenario for galaxy bias modelling.    
\end{itemize}

We run our MCMC chains with all combinations of the optimistic and pessimistic priors on intrinsic alignment, photo-$z$ biases and shear multiplicative bias. The results of this analysis is presented in Table \ref{tbl:sys_priors} and Figure \ref{fig:priors_plot}. In that table and figure, we present the dark energy figure-of-merit for the different combinations of optimistic and pessimistic priors. As we can see, shear multiplicative bias does not impact the results even if we are only able to determine it at a $\sim 1\%$ level (twice the value of DESC-SRD). 
On the other hand, strongly constraining IA and photo-$z$ biases can lead to stronger constraints on cosmological parameters.  
For the pessimistic scenario in $\Delta_z$, the dark energy figure-of-merit is degraded by $\sim 20\%$ (for Y1) to $\sim 40\%$ (for Y10). Similarly, constraining IA better by a factor of 2 (optimistic scenario for IA) leads to an improvement in FoM of $\sim 30$-$40\%$. When considering the optimistic scenario for both IA and photo-$z$, this leads to an improvement of over 50$\%$ for LSST-Y1 and almost $100\%$ improvement for LSST-Y10. These results show the value of being able to strongly constrain photo-$z$ biases and intrinsic alignment in improving the cosmological constraints. In particular, it shows the value of future spectroscopic surveys \citep{Astro2020_spectroscopy1, Astro2020_spectroscopy2, Snowmass, megamapper} to enhance the cosmological returns from LSST. 



==> sections_deprecated/intro.tex <==
\section{Introduction}\label{sec:intro}

The upcoming Vera Rubin Observatory's Legacy Survey of Space and Time \citep[LSST\footnote{\url{https://www.lsst.org/}},][]{LSST2019} will be part of a new era of cosmological surveys aimed at uncovering the nature of dark energy. Along with other Stage-IV surveys \citep{DETFreport2006} like Euclid \footnote{\url{https://sci.esa.int/web/euclid}} \citep{laa11}, the Nancy G. Roman Space Telescope \citep[NGRST\footnote{\url{https://roman.gsfc.nasa.gov/}},][]{sgb15}, and the Dark Energy Spectroscopic Instrument \citep[DESI \footnote{\url{https://www.desi.lbl.gov/}}][]{DESI16}, LSST will examine the nature of dark energy with an exquisite precision. Among the various probes of dark energy in LSST, multiprobe cosmological analyses with weak lensing, galaxy-galaxy lensing, and galaxy clustering, commonly referred to as `3$\times$2', will provide one of the strongest constraints on the dark energy parameters \citep{DESC_SRD}.
% through various cosmological probes, such as Type Ia supernovae, weak and strong lensing, and galaxy clusters. The cosmological analysis of these data sets are expected to be limited by our understanding of different systematic effects. As such, a significant challenge in analyzing these surveys is to make sure the results are robust against these effects.


However, weak lensing and galaxy clustering measurements are strongly impacted by various systematic effects \citep{Mandelbaum2018}. The impact of systematic effects is mitigated through various strategies, for example, by cutting out relevant scales where the modeling is imprecise or by including additional `nuisance' parameters in the model. While these mitigation schemes can reduce the bias on cosmological parameters, using an aggressive scale cut or an overly flexible systematics model leads to a loss in constraining power. As a result, bias-variance tradeoff is at play when deciding our analysis choices that are applied to the actual dataset and mapping out different aspects of this tradeoff is crucial as we prepare for LSST data analysis. Such an exercise will allow us to prioritize algorithmic development or future observational efforts to mitigate the systematic effects most important for our cosmological analysis. Identifying priorities for systematics mitigation strategy is the objective of this paper.

The analysis choices for the Stage-III survey cosmic shear and multiprobe analyses are determined using the full data analysis pipeline to ensure that the results are robust to known systematic effects \citep[e.g.][]{Hikage2019, Heymans2021, Krause2021}. These impact studies require hundreds to thousands of computationally expensive MCMC chains. Furthermore, the process needs to be repeated for each new probe or analysis. For Stage-IV survey data analysis, this challenge will become computationally even more expensive mostly because of the more complex systematics models that consequently span a larger parameter space. While simulated likelihood analysis with the full analysis pipeline is the most correct way to perform these impact studies, it is a serious computational bottleneck for future Stage-IV surveys. As such, we need robust forecasting pipelines that can perform fast, yet accurate inference.     

% \iffalse
Fisher matrix formalism is a common technique for fast forecasting, but it assumes that the posterior can be described as a multivariate Gaussian \citep{Wolz2012} and it can show numerical instabilities in high dimensions \citep{Euclid2020, Bhandari2021, YahiaCherif2021}. Alternate proposals for fast cosmological analyses include analytically marginalizing subsets of the full parameter space \citep{Hadzhiyska2020,Stolzner2021, Hadzhiyska2023, RuizZapatero2023} or importance sampling but these methods too rely on the assumption that the impact of marginalized parameters on the data vectors can be linearized, which may not be suitable for non-linear systematics models. Importance sampling is another approach frequently used for quick impact studies, but it only works close to the already sampled parameter space and it becomes problematic in high dimensional parameter spaces with with degeneracies. 


Machine-learning based emulators that are trained on the specific analysis pipeline are emerging as a computationally efficient and accurate avenue to predict the data vectors. However, standard emulator designs struggle to perform well in high-dimensions due to the curse of dimensionality. To circumvent this problem, iterative emulators have been proposed in the literature \citep{To2023, Boruah2022, Nygaard2022, Paranjape2022} where training points are acquired from a previous iteration of sampling. In this paper, we use the emulator introduced in \citet{Boruah2022} to extensively study different aspects of 3$\times$2 analysis with LSST. This method can perform accurate emulation in the high-dimensional parameter spaces of Stage-IV surveys such as LSST at a fraction of the computational cost of running the full pipeline. While we focus on LSST in this paper, our emulator provides a framework for undertaking the impact studies in preparation for any future photometric surveys such as Roman Space Telescope and Euclid. 


% In this paper, we will focus on multiprobe cosmological analysis using weak lensing, galaxy-galaxy lensing, and galaxy clustering, commonly referred to as `3$\times$2 point analysis'. 3$\times$2 pt analysis is forecasted to provide some of the strongest constraints on dark energy parameters for LSST among all cosmological probes \citep{DESC_SRD}. 

In this paper we study the impact of marginalization over different systematic effects closely following the Dark Energy Science Collaboration Science Requirement Document \citep[][DESC-SRD from hereon]{DESC_SRD}. The main differences differences/updates compared to the DESC-SRD are: 1) Our simulated likelihood analyses uses emulator-based MCMC runs, while the DESC-SRD uses Fisher matrix, 2) our data vector is comprised of real space angular correlation functions, while DESC-SRD performed its analysis is Fourier space, 3) we also marginalize over baryonic physics uncertainties, and 4) we chose a different lens sample and tomographic binning.

With respect to the latter point, the DESC-SRD uses the LSST Gold sample as the lens sample, whereas we we perform a `lens=source' analysis where the source sample itself is used as the lens sample. Such analyses have been previously considered in \citep{Schaan2020, Fang2022} and are motivated by the idea using one galaxy sample reduces the number of systematic parameters in a likelihood analysis. For example, \citet{Fang2022} show an increase in the signal-to-noise of the data vectors and stronger self-calibration of the redshift distribution when going from the `standard' analysis to the `lens=source' analysis.

This paper is structured as follows: After describing the theoretical basics and LSST survey assumptions in section \ref{sec:background} and Section \ref{sec:survey} we move to the main goal of this paper, i.e. exploring the `systematic error budget' of our baseline 3x2 analyses as a function of survey progress of LSST (Y1, Y3, Y6, Y10). Specifically, we quantify how much cosmological constraints weaken when marginalizating over (combinations of) different systematic effects and when assuming different priors on the systematics parameters (section \ref{sec:science_return_map}). In section \ref{sec:small_scales} we examine the gain in cosmological information when including small scales through improved baryonic and galaxy bias models. Finally, we explore the impact of photo-z outliers for LSST 3x2 analyses in section \ref{sec:photoz_outliers} before concluding in section \ref{sec:summary}.


==> sections_deprecated/photoz_outliers.tex <==
% \newpage

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/photoz_outliers/cosmo_contours_outliers.pdf}
    \caption{Impact of inaccurate determination of photo-$z$ outlier fractions on cosmological constraints with LSST-Y10 mock survey. For each of the analysis shown here, the model assumes the outlier fraction to be 0.02. But the simulated data vector is computed assuming an outlier fraction of 0.015 (blue contours), 0.02 (red contours) and 0.025 (grey dashed contours). As can be seen from the figure, inaccurate determination of the outlier fraction can lead to highly biased inference of the cosmological parameters.}
    \label{fig:outliers_contour_plot}
\end{figure}


\section{LSST synergies with spectroscopic datasets}\label{sec:spectro}

\subsection{Impact of catastrophic photo-$z$ outliers}\label{ssec:photoz_outliers}

In previous sections, we assumed that uncertainty in the photometric redshift distributions for the tomographic bins can be accurately captured with just a constant shift. However, due to type-redshift degeneracy, some of the redshifts are mis-estimated by $\mathcal{O}(1)$, commonly known as catastrophic redshift outliers. If these outliers are not properly addressed in the analysis, they can significantly skew the results of cosmological studies for Stage-IV surveys \citep{Sun2009, Bernstein2010, Hearin2010, Schaan2020, Fang2022}.

In this section, we examine the effects of these catastrophic outliers on cosmological constraints. There are various methods to mitigate the impact of photometric redshift outliers in 3$\times$2 point analysis. For instance, the fraction of outliers in the sample can be determined using spectroscopic observations \citep{Sun2009, Bernstein2010}. 
By conducting impact studies, we determine the level of accuracy required in determining the outlier fraction to ensure that the cosmological analysis is not significantly biased. We apply this analysis to our mock surveys for LSST-Y1/Y10. The results of these analyses can be used to establish the spectroscopic requirements for a reliable cosmological analysis with LSST. Note that in this analysis, we do not add any extra parameters to address the impact of photometric redshift outliers. These results may differ if we use mitigation schemes to self-calibrate the fraction of outliers in the analysis \citep[e.g,][]{Schaan2020, Fang2022}.

 To conduct our impact studies, we use a mock galaxy sample created by \citet{Graham2018} that includes a population of catastrophic outliers. We fit a multivariate Gaussian to the joint probability distribution, $p_{\text{out}}(z_{\text{true}}, z_{\text{phot}})$, of the outlier sample and add it to the analytic distribution (equation \eqref{eqn:smail}) with varying outlier fractions. Then, we train an emulator with an outlier fraction of $2\%$ and create a set of simulated data vectors with different outlier fractions. Finally, we analyze these simulated data vectors with the emulator and determine the accuracy required to estimate the outlier fraction to get robust cosmological constraints. This can be used to set requirements on the spectroscopic needs for LSST \citep{Sun2009, Bernstein2010}. It's worth noting that we do not consider cross-correlations between different redshift bins and the effect they may have on self-calibrating photo-z outliers \citep{Schaan2020}.

The results of our analysis are displayed in Figures \ref{fig:outliers_contour_plot} and \ref{fig:outliers_tolerance}. Figure \ref{fig:outliers_contour_plot} illustrates the impact on cosmological constraints if the fraction of outliers is mis-estimated in the analysis. The figure shows that a mis-estimation of the outlier fraction can result in significant biases in the cosmological constraints. In particular, the $w_0$-$w_a$ plane can be significantly impacted. Figure \ref{fig:outliers_tolerance} shows the bias in the $w_0$-$w_a$ plane for varying levels of mis-estimation in the outlier fraction for LSST-Y1 and LSST-Y10 mock surveys. The figure demonstrates that in order to ensure that the cosmological constraints are not shifted by more than $0.3\sigma$ ($0.5\sigma$), the outlier fraction must be determined to an accuracy of $0.001~(0.002)$ for LSST-Y10 (Y1), or a $5\%(10\%)$ determination of the outlier fraction. Thus, it puts stringent constraints on the accuracy with which the outlier fraction should be known in order to ensure robust cosmological constraints using LSST 3$\times$2 point analysis.  

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/photoz_outliers/outlier_fraction.pdf}
    \caption{Bias in the $w_0$-$w_a$ parameters as a function of difference in the assumed outlier fraction for the LSST-Y1 (red circles) and LSST-Y10 (green circles) mock surveys. The dashed and dotted black lines corresponds to $0.3\sigma$ and $0.5\sigma$ bias in the $w_0$-$w_a$ plane. As we can see from the figure, in order to achieve cosmological inference with less than $0.5\sigma$ bias, we need to determine the outlier fraction to within $5\%$ ($10\%$) accuracy for LSST-Y10 (Y1).}
    \label{fig:outliers_tolerance}
\end{figure}


\subsection{Low-$z$ spectroscopic survey for improved IA}\label{ssec:lowz_specz}

There have been proposals to extend the current spectroscopic surveys, such as DESI, to produce a high-density spectroscopic galaxy sample at $z < 1$ \citep[e.g,][]{Schlegel2022}. In this section, we investigate the utility of such a survey for mitigating LSST systematics at low redshift. Specifically, data from such a survey can be used to directly measure intrinsic alignment through position-shape cross-correlations \citep{Singh2015, Samuroff2022}. Following \citet{Krause2016}, we investigate the impact of intrinsic alignment at low-$z$ on 3$\times$2 pt analysis.  

The results of this impact study is shown in Figure \ref{fig:lowz_ia}. In this analysis, we first create a synthetic data vector which contains intrinsic alignment contribution and analyze it using a model with no IA. As we can see from the figure, ignoring IA in the analysis leads to a large bias in the cosmological constraints (blue contours in Figure \ref{fig:lowz_ia}). With a dense low-$z$ spectroscopic sample, we will be able to model the intrinsic alignment at low-$z$. To mimic this scenario, we create a synthetic data vector, where we assume that IA has been perfectly modeled and subtracted off at $z < 1$. This is achieved by setting the $II$ and $GI$ term of the power spectrum to zero at $z < 1$ while calculating the data vector. When we analyze this data using a model with no intrinsic alignment, we see no significant bias (red contours in the Figure), showing that the presence of intrinsic alignment at high-$z$ does not impact the cosmological constraints. For comparison, the grey contours show the results of a self consistent model run, where both the model and data vector has no IA contamination. These results confirms the results of \citet{Krause2016} that modelling the IA contamination at $z < 1$ leads to robust cosmological analysis. On the other hand, unmodelled IA at high redshifts ($z > 1$) does not significantly impact the 3$\times$2 pt cosmological analysis. In reality, IA cannot be modelled perfectly as assumed here. We leave detailed quantitative exploration of this assumption to a later work. But these results strengthens the case for a dense low-$z$ spectroscopic sample as a way to mitigate intrinsic alignment mitigation in LSST 3$\times$2 point analysis.


While not shown here, we also investigate the impact these low-$z$ surveys can have on LSST 3$\times$2 pt analysis by better constraints on $\Delta_z$ at low redshifts. We find that better constraints on $\Delta_z$ can only marginally improve the cosmological constraints -- it leads to $\mathcal{O}(5\%)$ improvement in $w_0$-$w_a$ FoM. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/lowz_ia/ia_run_contaminated_dv.pdf}
    \caption{Impact of not modeling intrinsic alignment on cosmological constraints from LSST-Y1 3$\times$2 pt analysis. In all the three analyses, we ignore intrinsic alignment in the model. The blue contours show the analysis of a data vector that contains no intrinsic alignment contamination. The analysis of data vectors with IA contamination is shown with grey-dashed contours. As we can see, ignoring IA leads to large biases in the cosmological constraints. However, if we are able to perfectly model IA at $z < 1$ (mimicked by having IA contamination in the data vector only at $z > 1$), the resulting cosmological constraints are no longer biased (red contours). This result shows the value of a low-$z$ spectroscopic survey for mitigating IA in LSST analysis.}
    \label{fig:lowz_ia}
\end{figure}

% \newpage

==> sections_deprecated/small_scales.tex <==
\begin{figure*}
    \centering
    % \includegraphics[width=0.8\linewidth]
    % {figs/error_budget/small_scales/y3_3pcas.pdf}
    \includegraphics[width=\linewidth]{figs/error_budget/small_scales/corner_plot_y3.pdf}
    
    \caption{Constraints on cosmological and baryonic physics parameters obtained with LSST-Y3 3$\times$2 pt analysis using the fiducial scale cut (red-dashed), a more conservative scale cut twice the fiducial scale cut (blue) and the 1 arminute scale cut (grey). As we can see, pushing the analysis to smaller scales do not improve the cosmological constraints significantly. On the other hand, the constraints on the baryonic physics parameters improve dramatically. The darker and lighter regions in the contours correspond to the 68 and 95 percent confidence intervals. }
    \label{fig:contour_plots_scalecut}
\end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figs/baryonic_physics/baryon_constraints.pdf}
%     \caption{Constraints on baryon PC parameters for three hydrodynamical simulations - BAHAMAS-T7.6 (red), BAHAMAS-T8.0 (orange), and Eagle (blue) - analyzed using a 1 arcminute scale cut for cosmic shear. The markers on the plot represent baryon PC parameters obtained from data vectors of different hydrodynamical simulations. The four columns correspond to the analysis for the LSST-Y1/Y3/Y6 and Y10 mock surveys. This plot demonstrates the power of small-scale cosmic shear in providing valuable information on baryonic physics, as it enables us to distinguish between different hydrodynamical simulations, even at the precision of LSST-Y1.}
%     \label{fig:baryonic_physics_constraints}
% \end{figure*}

\section{Including small scales in 3$\times$2 point analysis}\label{sec:small_scales}

Our ability to model small scales in 3$\times$2 point data vector is limited by our incomplete understanding of baryonic physics and non-linear galaxy bias. To ensure that these systematic effects do not bias our cosmological results, typically the small scale measurements are discarded when performing 3$\times$2 point analysis. While discarding small scale data points ensures unbiased results, it also results in discarding meaningful cosmological information. To recover the lost information in 3$\times$2 pt analysis, there have been efforts to model the small-scale signature of baryonic physics \citep{Eifler2015, Huang2019, Mead2021} and galaxy bias \citep{Kokron2021, Salcedo2022}. In light of these efforts, it is useful to ask the question: how much information is recovered by pushing the analysis to small scales? In section \ref{ssec:small_scale_info}, we consider this question and quantify the information gained by pushing 3$\times$2 point analysis to small scales.

In spite of these efforts, no model will be perfect on small scales and we will need to discard certain scales on small scales. Therefore, an essential step in preparing for the 3$\times$2 pt analyses from a cosmological survey is to determine the optimal scale cuts where the cosmological returns are maximized, yet the results are unbiased. These scale cuts are typically determined by performing impact studies, where a contaminated data vector is analyzed using an incomplete data model. If the resulting bias is above some pre-determined threshold, we repeat the analysis by discarding more data points on small scales. This requires us to run a large number of these analyses - which are computationally intensive using the traditional methods, but is extremely fast with our data vector emulator. This is considered in section \ref{ssec:impact_studies}, where we show how we can use our data vector emulator to perform fast impact studies.

Typically, the scale cuts for cosmic shear and GGL/galaxy clustering are chosen differently, as baryons are the main contaminant for cosmic shear and non-linear galaxy bias is the main contaminant for GGL/galaxy clustering. The scale cuts for cosmic shear are usually set at a specific angular scale, as lensing kernels are affected by all matter along the line-of-sight.\footnote{Although see \citet{Taylor2018, Taylor2021} for an alternate approach}
The scale cuts for GGL/galaxy clustering, on the other hand, are defined in physical scales. This approach is followed in this section.

\subsection{Information gain on small scales}\label{ssec:small_scale_info}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/error_budget/small_scales/fom_npcas_scalecuts.pdf}
%     \caption{Dark energy figure-of-merit for the simulated runs as a function of number of PCA modes marginalized. The solid lines corresponds to the runs with the DESC-SRD scale cuts and the dotted lines correspond to the result with the 1 arcminute scale cuts. As can be seen from the figure, the dark energy figure of merit does not change substantially either when we analyze with smaller scale cuts (comparing the solid lines with the dotted lines) or if we marginalize over more baryonic parameters (the points on the same curve are of similar magnitude).}
%     \label{fig:fom_vs_npcas}
% \end{figure}

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/error_budget/small_scales/fom_smallscales.pdf}
    \caption{Dark energy figure of merit for LSST-Y1 (red circles), Y3 (black triangles), Y6 (blue hexagons) and Y10 (orange star) mock surveys at various scale cuts for GGL and galaxy clustering. As we can see, we can gain a lot of cosmological information by pushing the analysis to smaller scales. Note however that here we have assumed linear bias in our data vectors -- an assumption that will break on small scales. Therefore the information gain here should be thought of as the potential ceiling.}
    \label{fig:galaxy_small_scales}
\end{figure}
\fi

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/baryonic_physics/baryons_impact_bias.pdf}
    \caption{Impact of baryonic feedback on cosmological analysis for LSST Y1/Y3/Y6 and Y10 mock surveys. We plot the marginalized 1D posteriors of the cosmological parameters $\Omega_m$, $n_s$, $w_0$, $w_a$ for our analysis of the contaminated data vectors with varying number of baryon PCA modes used to account for baryons. The true parameter values are denoted with the black dashed lines. As we can see, without marginalizing over the baryon feedback parameters, the resulting cosmological parameters are heavily biased. However, marginalizing over 1/2 PCA modes is sufficient to capture the impact of most small-scale baryon feedback scenarios.}
    \label{fig:baryon_impact_study}
\end{figure*}

In this section, we quantify the possible information gain when pushing 3$\times$2 pt analysis to small scales. To analyze the small scale information in cosmic shear, we consider scale cuts that are much smaller (upto 1 arcminute) than the fiducial scale cuts for $\xi_{\pm}$. To analyze the small scale information in GGL and galaxy clustering, we consider pushing the analysis to scale cuts of $4/8/12/16~h^{-1}$ Mpc. Since the goal of this section is to simply quantify the information gain on small scales, our synthetic data vector do not contain the effects of baryons and non-linear bias on small scales. The impact of these small-scale systematics is considered in section \ref{ssec:impact_studies}, where we show how we can use our emulator for fast impact studies for 3$\times$2 pt analysis.

\iffalse
The first metric we use to quantify the information gain at different scale cuts is the signal-to-noise ratio (SNR) for the synthetic data vectors at different scale cuts. The SNR is defined as, 
\begin{equation}
    \text{SNR} = \sqrt{\mvec{d}^{\text{T}}\mmat{C}^{-1}\mvec{d}}.
\end{equation}
The SNR is routinely used to analyze the information gain and it reflects the size of the signal in the data vector relative to the covariance. The SNR for LSST-Y1/Y3/Y6/Y10 mock surveys for the different scale cuts is shown in Table \ref{tbl:snr}. We can see from that table that the SNR increases substantially as we go to smaller scales in both the cosmic shear part of the data vector as well as the GGL and the galaxy clustering part of the data vector.

While the SNR is useful for preliminary assessment of the information gain, due to non-linear dependence of the data vectors on different cosmological and systematics parameters and non-trivial degeneracies between different parameters, the SNR does not necessarily translate to constraints on different parameters in a simple way. 
\fi

In order to analyze the information gain on small scales, we run our MCMC chains including full data realism. Usually such analyses are limited by the intensive computation required for the full analysis. But since in our emulator, we emulate the data vector on all scales, we can perform quick analysis by simply switching the scale cuts used in the analysis. We therefore use our emulator-based analysis for fast, yet precise forecasts of the information gained by pushing the analysis to small scales. 

As our first example, we run MCMC chains with three scale cuts on $\xi_{\pm}$: the fiducial scale cuts defined in section \ref{ssec:scale_cuts}, a much smaller 1 arcminute scale cut and a more conservative scale cut that is twice the fiducial scale cuts. Pushing the analysis from the fiducial scale cuts to a much smaller 1$^{\prime}$ results in a substantial increase in the SNR for each of the LSST mock surveys (e.g, it goes from $426$ to $462$ for LSST-Y10). This shows that there is potentially a lot of information to be gained by pushing the analysis to smaller scales. The question remains how this information translates to constraints on different parameters. The results from our simulated analyses are presented in Figure \ref{fig:contour_plots_scalecut}, where we plot the contours obtained for the cosmological and baryonic physics parameters for the runs with the three scale cuts for the LSST-Y3 mock survey. From the figure we see that there is almost no improvement in cosmological constraints by pushing the analysis to smaller scales. On the other hand, the constraints on the baryonic PC parameters improves immensely by pushing the analysis to small scales (shown in the upper right panels of Figure \ref{fig:contour_plots_scalecut}). This suggests that by utilizing the small-scale information from 3$\times$2 pt analysis, we will be able to improve the constraints on baryonic physics dramatically. Such analyses have been performed by multiple groups to constrain the signature of baryonic feedback on small scales. For example, \citet{Huang2021} analyzed the DES-Y1 data to put constraints on baryonic physics using 3$\times$2 pt analysis. More recently, \citet{Amon2022, Preston2023} analyzed the cosmic shear data from KiDS and DES-Y3 using a simple one-parameter model to find strong signatures of baryonic feedback and \citet{Chen2023, Arico2023} used small-scale measurements from DES-Y3 to put strong constraints on baryonic physics parameters. We forecast the power of small-scale analyses to constrain baryonic physics with 3$\times$2 point analysis with our LSST mock surveys in Figure \ref{fig:baryonic_physics_constraints} where we analyze the simulated data vectors that contain baryonic physics contaminations from various hydrodynamical simulations. In that figure, we show the results of running our analysis with a 1 arcmin scale cut for $\xi_{\pm}$ on the data vectors from three hydrodynamical simulations - BAHAMAS-T7.6, BAHAMAS-T8.0 and Eagle. Also shown are the baryon PC amplitudes measured for a number of hydrodynamical simulations. From the figure we see that by utilizing the small-scale information, we will be able to constrain baryonic physics with exquisite precision. Already at the precision of LSST-Y1 precision, we will be able to rule out most of the hydrodynamical simulation scenarios. This suggests that improved baryonic physics modeling may be required to utilize the full information from LSST 3$\times$2 pt data.


Furthermore, marginalization over baryonic physics has little impact on the dark energy figure-of-merit for either of the scale cuts. This is reflected in Figure \ref{fig:fom_vs_npcas} where we plot the dark energy Figure-of-merit as a function of the number of PCA modes marginalized in the analysis for the 4 LSST years considered. This is to be expected from the results of Figure \ref{fig:systematics_error_budget}, where we already show that marginalization over the baryonic physics parameters has little impact on the dark energy figure-of-merit. It thus also follows that marginalizing over the baryonic physics parameters does not degrade the cosmological constraints. 

% We also investigate the information gain obtained by pushing the 3$\times$2 pt analysis to smaller scales for the GGL and galaxy clustering part of the data vector. We run chains for scale cuts corresponding to $4/8/12/16~h^{-1}$ Mpc. The results of this analysis are shown in Figure \ref{fig:galaxy_small_scales} where we show the DE FoM for the analysis at different galaxy scale cuts. Unlike the analysis for cosmic shear small scales, we can see from the figure that pushing to smaller scales can lead to substantial gain in the constraints on cosmological parameters. We however note that for this analysis, our synthetic data vectors are created assuming linear bias, which breaks down on the scales considered here. Therefore, this information gain should be regarded as a ceiling for the possible information gain. It is possible that marginalizing over the non-linear bias parameters will wash out some of the gain in cosmological parameters. Investigating the impact of higher-order bias parameters is deferred to a later work. 

% \iffalse
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/galaxy_bias/impact_study_galaxy_bias.pdf}
    \caption{Impact of non-linear galaxy bias on cosmological constraints. When analyzing linear bias data vector with a linear galaxy bias model (shown in red), there are no biases in the inference. Note however that due to projection effects, the resulting 1D posteriors are not centred on the fiducial values. However, when analyzing the data vector containing non-linear galaxy bias with a linear bias model (shown in blue), cosmological constraints are significantly biased at small scale cuts.}
    \label{fig:galaxybias_impact_study}
\end{figure*}
% \fi

\subsection{Impact studies}\label{ssec:impact_studies}
% \iffalse
In the previous section, we looked at the potential information gained by pushing 3$\times$2 pt analyses to smaller scales. However, pushing these analysis to smaller scales will make the impact of baryons and non-linear galaxy bias worse. In order to ensure that the cosmological constraints obtained in our analysis are unbiased, we need to perform `impact studies' where we analyze synthetic data vectors containing the effects of known systematics. These analyses help us study the impact of different systematics on the cosmological constraints. Such impact studies are an essential part of preparing for the analysis of cosmological surveys to define optimal analysis choices such as scale cuts and systematics modelling \citep[e.g,][]{Krause2021, Heymans2021}. This requires us to run multiple MCMC chains which can be computationally intensive with traditional methods. Furthermore these types of analyses needs to be repeated for new physics models and new probes. 

In this section, we show how our data vector emulator can be used to massively speed up this process. We show two examples, where we show the impact of baryons and non-linear galaxy bias on the cosmological constraints from 3$\times$2 pt analysis. Note that the emulator we use in this work is designed to work only in the high-posterior region of the parameter space. Therefore, the exact amount of bias incurred may not be trustworthy. However, these impact studies are used to identify the modeling choices so that the posterior shifts are below certain thresholds. Hence, these points of parameter space are still within the emulator training range and therefore the results are still trustworthy.  

As a first example, we look at the impact of baryons on cosmological constraints when analyzing the results with the optimistic scale cut of 1 arcmin. The results of this analysis are presented in Figure \ref{fig:baryon_impact_study}, where we plot the marginalized 1D posteriors of the cosmological parameters ($\Omega_m$, $n_s$, $w_0$, $w_a$) of the analysis with data vectors contaminated with baryonic scenarios of different hydrodynamical simulations. We analyze the data vectors with varying number of baryon PCAs. As we can see, for most of the baryonic scenarios, marginalizing over 2 or 3 PCA modes is sufficient to marginalize over the small-scale baryonic effects. We note however that there is some residual bias when analyzing the Illustris data vector, which is not used in calculating the principal component. 


For our second example of impact study, we study the impact of non-linear galaxy bias on 3x2 point analysis. In these simulated analyses, we assume linear bias in our model, but the simulated 'observed' data vector is computed using non-linear bias. We compute the impact of non-linear bias using perturbation theory \citet{Pandey2020}. In our simulated data vector, the second order bias parameter, $b_2$, is calculated in terms of the linear bias parameter, $b_1$, using the fitting formula of \citet{Lazeyras2016}. The tidal and the third-order bias term is set to their co-evolution values \citep{Saito2014, Pandey2020}. We analyze these data vectors for $4$ different scale cuts ranging from 4$h^{-1}$ Mpc to 16$h^{-1}$ Mpc. The results of these analyses are shown in Figure \ref{fig:galaxybias_impact_study}. As can be seen from the Figure, analyzing the non-linear galaxy bias data vector with linear bias model leads to substantial bias in the 1D posteriors for scale cuts $\lesssim 8~h^{-1}$ Mpc for all of the years of LSST considered.  
\cyan{With this analysis we verify that the scale cuts assumed in DESC-SRD is sufficient to mitigate the impact of non-linear bias.}















==> sections_deprecated/summary.tex <==
\section{Discussion and Summary}\label{sec:summary}

Running MCMC chains to perform cosmological inference is a significant computational bottleneck for performing 3$\times$2 point analysis. This problem will likely be worse for 3$\times$2 pt analyses with Stage-IV surveys due to more complex modeling. To circumvent this problem, we introduced an iterative neural network based emulator design in \citet{Boruah2022}. The emulator allows us to run fast 3$\times$2 pt analysis while maintaining the realism of the full data analysis pipeline. In this paper, we used this emulator to perform such `precision forecasting' for `lens = source' 3$\times$2 point analysis with LSST. Using the emulator allows us to run hundreds of simulated likelihood analyses for LSST-Y1/Y3/Y6 and Y10 mock surveys while using much lower computational resources. We map out the information content and the impact of different systematic effects on cosmological parameter inference. Using this high-level cosmology inference can inform decision making by prioritizing research on systematic mitigation and deciding various analysis choices. While the specific results obtained in this paper will likely change depending on different analysis choices, the methodology described here is applicable for all future analyses. 

Here, we investigated the systematic error budget of 3$\times$2 pt analysis, i.e, the contribution of marginalizing over different systematic parameters on the overall error budget. We find that marginalizing over the galaxy bias parameters contributes the most to the overall cosmological error budget. On the other hand, marginalizing over the baryonic or shear multiplicative bias parameters do not contribute significantly to the overall error budget. Furthermore, we find that strong constraints on $\Delta_z$ and IA parameters  can improve the dark energy figure-of-merit by $30$-$40\%$, showing the value of future spectroscopic surveys in the LSST footprint.

We also investigate the gains in information content by pushing the analysis to smaller scales. We find that utilizing the small scale cosmic shear does not improve the cosmological constraints significantly. However, the small scale cosmic shear leads to improved constraints on baryonic physics.  

Another aspect of 3$\times$2 point analysis that we examine is the determination of optimal modelling choices so that cosmological constraints are robust to small-scale systematics like baryons and non-linear galaxy bias. In section \ref{ssec:impact_studies}, we illustrated how our emulator-based analysis can accelerate fast impact studies that are important for determining modeling choices such as scale cuts. Determining the optimal scale cuts involve running many MCMC chains so that with different scale cuts. Because we train our emulator to predict the 3$\times$2 point data vector at all scales, we can run fast MCMC analysis with different scale cuts, thus reducing greatly the computational cost involved in these impact studies.   
     

Finally, we also studied the impact of catastrophic photo-$z$ outliers on cosmological parameter inference. Catastrophic outliers are galaxies for which the photometric redshifts are mis-estimated by $\gtrsim \mathcal{O}(1)$. Photo-$z$ outliers can significantly impact cosmology inference for $3\times2$ pt analysis \citep{Bernstein2010, Fang2022}. In this paper, we studied the impact of mis-estimating the photo-$z$ outlier fraction on bias in cosmological parameters. We find that the outlier fraction needs to be determined to within $5\%$ ($10\%$) accuracy to ensure unbiased inference of dark energy. Such analyses can be used to put requirements on the spectroscopic needs for photo-$z$ estimation.

Our emulator based method gives a way to propagate the impact of various systematics modeling to the high-level cosmological analysis in a fast way, while maintaining full data realism. 

==> sections_deprecated/survey.tex <==

\begin{figure*}
    \includegraphics[width=\linewidth]{figs/lsst_nz_diff_years.pdf}
    \caption{The redshift distribution, $n(z)$, for the LSST Y1/Y3/Y6/Y10 mock LSST surveys. The redshift distribution is generated according to the analytical distribution given in equation \eqref{eqn:smail} and then divided into $10$ tomographic bins with equal number of galaxies in each bin. The parameters $z_0, \alpha$ are given in Table \ref{tbl:survey_conf}.}
    \label{fig:lsst_nz}
\end{figure*}

\section{Survey assumptions and modeling choices}\label{sec:survey}


\begin{table}
  \centering
  \caption{Survey configurations for our mock LSST-Y1/Y3/Y6/Y10 surveys. $n_{\text{eff}}$ denotes the effective number density of the source sample. $z_0, \alpha$ are the parameters controlling the redshift distribution given in equation \ref{eqn:smail}. $\sigma_e$ and $\sigma_z$ denotes the shape noise and the photo-$z$ scatter respectively.}
  \begin{tabular}{l c c c c}
  \hline
     Parameter &  LSST-Y1 & LSST-Y3 & LSST-Y6 & LSST-Y10\\
    \hline
    Area & $12300$ & $12744$ & $13411$ & $14300$\\
    $n_{\text{eff}}$ & $10.47$ & $16.75$ & $22.52$ & $27.10$\\    
    $z_0$ & $0.193$ & $0.184$ & $0.179$ & $0.176$ \\
    $\alpha$ & $0.876$ & $0.828$ & $0.800$ & $0.783$ \\
    $\sigma_e$ & $0.26$ & $0.26$ & $0.26$ & $0.26$ \\
    $\sigma_z$ & $0.05$ & $0.05$ & $0.05$ & $0.05$ \\
    \hline
  \end{tabular}
  \label{tbl:survey_conf}
\end{table}

\begin{table*}
  \centering
  \caption{Fiducial value and the prior used on various cosmological and systematic parameters. In the table flat$[a,b]$ denotes a flat prior between $a$ and $b$, whereas Gauss$[\mu, \sigma^2]$ denotes a Gaussian prior with mean $\mu$ and standard deviation $\sigma$. See section \ref{ssec:systematics} for more detail on the modelling of the systematic parameters.}
  \begin{tabular}{l c c c c c}
  \hline
     Parameters &  Fiducial & LSST-Y1 Prior & LSST-Y3 Prior & LSST-Y6 Prior & LSST-Y10 Prior\\
    \hline
    \textbf{Cosmology} & & \\
    $\omega_\textrm{c}$ & $0.1274$ & flat$[0.01, 0.3]$ & flat$[0.01, 0.3]$ & flat$[0.05, 0.25]$ & flat$[0.05, 0.25]$\\
    $\log (A_\textrm{s} \times 10^{10})$ & $3.04452$ & flat$[2.5, 3.5]$ & flat$[2.5, 3.5]$ & flat$[2.65, 3.4]$ & flat$[2.65, 3.4]$\\
    $n_{\textrm{s}}$ & $0.97$ & flat$[0.87, 1.07]$ & 
    flat$[0.87, 1.07]$ & 
    flat$[0.91, 1.04]$ & 
    flat$[0.91, 1.04]$ \\
    $\omega_\textrm{b}$ & $0.0196$& flat$[0.01, 0.04]$ & flat$[0.01, 0.04]$ & flat$[0.01, 0.04]$ & flat$[0.01, 0.04]$\\
    $h$ & $0.70$& flat$[0.60, 0.80]$ & flat$[0.60, 0.80]$ & flat$[0.60, 0.80]$ & flat$[0.60, 0.80]$\\
    \hline
    \textbf{Intrinsic Alignment} & & \\
    $a_{\ia}$ & $0.5$ & flat$[-5, 5]$ & flat$[-5, 5]$ & flat$[-5, 5]$ & flat$[-5, 5]$\\
    $\eta_{\ia}$ & $0$ & flat$[-5, 5]$ & flat$[-5, 5]$ & flat$[-5, 5]$ & flat$[-5, 5]$\\
    \hline
    \textbf{Linear galaxy bias} & & \\
    $b^{(i)}_1$&  & flat$[0.8, 3]$ & flat$[0.8, 3]$ & flat$[0.8, 3]$ & flat$[0.8, 3]$ \\
    \hline
    \textbf{Photo-$z$ bias} & & \\    $\Delta^i_{z,\text{source}}$ & 0 & Gauss$(0., 0.002^2)$ & Gauss$(0., 0.002^2)$ & Gauss$(0., 0.002^2)$ & Gauss$(0., 0.002^2)$\\
    \hline
    \textbf{Shear calibration} & & \\
    $m^i$ & 0 & Gauss$(0., 0.005^2)$ & Gauss$(0., 0.005^2)$ & Gauss$(0., 0.005^2)$ & Gauss$(0., 0.005^2)$\\
    \hline
    \textbf{Baryon PCA amplitude} & & \\
    $Q_1$ & 0 & flat$[-1000, 1000]$ & flat$[-1000, 1000]$ & flat$[-1000, 1000]$ & flat$[-1000, 1000]$\\
    $Q_2$ & 0 & flat$[-1000, 1000]$ & flat$[-1000, 1000]$ & flat$[-1000, 1000]$ & flat$[-1000, 1000]$\\
    $Q_{3}$ & 0 & flat$[-1000, 1000]$ & flat$[-1000, 1000]$ & flat$[-1000, 1000]$ & flat$[-1000, 1000]$\\
    \hline
  \end{tabular}
  \label{tbl:parameters}
\end{table*}

\subsection{LSST survey assumptions}\label{ssec:lsst_assumptions}

We closely follow the LSST-DESC SRD \citep{DESC_SRD} to design our Y1, Y3, Y6, and Y10 mock surveys. As specified in the DESC-SRD, we assume the Y1 survey area to be 12300 deg$^2$ and the Y10 survey area to be 14300 deg$^2$. We interpolate the areas of Y3 and Y6 linearly between Y1 and Y10, resulting in survey areas of 12744 deg$^2$ and 13411 deg$^2$ for Y3 and Y6, respectively. We note that survey optimization is an ongoing effort in LSST and that the final footprints will likely look differently. 

In this paper, we consider a "lens=source" analysis \citep[see e.g.][]{Fang2022} using the source sample as defined in the DESC-SRD also as the lens sample.

% The corresponding redshift distribution is obtained from the WeakLensingDeblending \footnote{\url{https://github.com/LSSTDESC/WeakLensingDeblending}} software-generated CatSim galaxy catalog. To obtain the redshift distribution for a given $i$-band depth, $i_{\text{depth}}$, this depth is applied to the input CatSim catalog and fit 
The resulting redshift distribution is fit to the parametric form  \citep{Smail1995},
\begin{equation}\label{eqn:smail}
    n(z) \propto z^2 \exp[-(z/z_0)^{\alpha}].
\end{equation}
The effective number density and the values of $z_0$ and $\alpha$ are obtained as a function of $i_{\text{depth}}$ which can be approximated using the following analytic formulae,

\begin{align}
    n_{\text{eff}} &= 10.47 \times 10^{0.3167 (i_{\text{depth}} - 25)} \\
    z_0 &= 0.193 - 0.0125 (i_{\text{depth}} - 25) \\
    \alpha &= 0.876 - 0.069 (i_{\text{depth}} - 25).
\end{align}
We assume that the LSST-Y1, Y3, Y6 and Y10 surveys will have $i_{\text{depth}} = 25.1, 25.7, 26.1, 26.35$ respectively. The resulting redshift distributions are convolved with a Gaussian photo-$z$ error of standard deviation, $\sigma_z = 0.05(1+z)$. The galaxies are then binned into $10$ tomographic bins of equal galaxy number density. The resulting redshift distributions are shown in Figure \ref{fig:lsst_nz} with effective number density for LSST-Y1/Y3/Y6 and Y10 being $n_{\text{eff}} = 10.47, 16.75, 22.52$ and $27.1$ arcmin$^{-2}$, respectively (also see Table \ref{tbl:survey_conf}). In section \ref{sec:photoz_outliers}, we will also consider the impact of photo-$z$ outliers, which changes the redshift distribution of the galaxies. 




\subsection{Systematics modelling}\label{ssec:systematics}

Our analysis includes observational systematic effects such as photo-$z$ uncertainties, shear biases and astrophysical systematics including baryons, intrinsic alignment and galaxy bias. 

\subsubsection{Photo-$z$}\label{sssec:photoz}

Inaccuracies in the photometric redshift distribution, $n^i(z)$ are modeled as a simple shift model that adds a new parameter, $\Delta^i_z$, to each tomographic bin, which shifts the redshift distribution as,
\begin{equation}
    n^i(z) \rightarrow n^i(z + \Delta^i_z). 
\end{equation} 
In "lens=source" analyses, we use the same $\Delta_z$ parameter for both the lens and source samples. This reduces the dimensionality of the parameter space, compared to using a different lens sample, and results in improved constraints on photometric redshift parameters and cosmological parameters \citep{Fang2022}. Our baseline analysis follows the DESC-SRD and assumes that the redshift distributions can be characterized with a precision of $0.2\%$ ($\sigma[\Delta_z] = 0.002$). In section \ref{ssec:priors}, we examine the impact of a more pessimistic photo-$z$ prior. Photo-z parameters are slow parameters that are included in the emulator training. 

\subsubsection{Baryons}\label{sssec:baryons}
Baryons impact matter distribution on small scales, which in turn affects the 3x2 observables. We use the formalism of \citet{Eifler2015, Huang2019} to account for the effects of baryons. In this formalism, we measure the changes in the matter power spectrum caused by baryonic physics in various hydrodynamical simulations.  In this paper, we use $8$ hydrodynamical simulations: Illustris TNG-100 \citep{Springel2018}, MassiveBlack-II \citep{Khandai2015}, Horizon-AGN \citep{Dubois2014}, 2 simulations (T8.0 and T8.5) of the cosmo-OWLS simulation suite \citep{LeBrun2014} and 3 simulations (T7.6, T7.8, T8.0) of the BAHAMAS simulation suite \citep{McCarthy2017}. 

We perform a Principal Component Analysis (PCA) to capture said difference as it affects our model vectors (equations  \eqref{eqn:xi_cosmic_shear}-\eqref{eqn:w_clustering}) with only a few modes. 
%Finally, we measure the modifications in the data vector caused by these principal components of the power spectrum at the fiducial cosmological parameters using the equations \eqref{eqn:xi_cosmic_shear}-\eqref{eqn:w_clustering} in section \ref{ssec:model_data_vector}. We denote these as $\text{PC}_i$.
% \red{We then measure the modifications in the data vector caused by the different hydrodynamical scenarios using the equations \eqref{eqn:xi_cosmic_shear}-\eqref{eqn:w_clustering} in section \ref{ssec:model_data_vector}. Finally, Principal Component Analysis (PCA) is performed on the modified data vectors to model the general effects of baryonic physics with only a few principal components. }
The the 3$\times$2 data vector including baryonic physics is then modeled in terms of the principal components $\text{PC}_i$ as,
\begin{equation}
    \mvec{d}_{\text{baryons}} = \mvec{d}_{\text{dmo}} + \sum_{i=1}^{N_{\text{PCA}}} Q_i \text{PC}_i,
\end{equation}
where $\{Q_i\}$, the amplitude of the $\text{PC}_i$, represent the additional nuisance parameters varied in a likelihood analysis and $\mvec{d}_{\text{dmo}}$ is the dark matter only data vector. In this paper, we use $N_{\text{PCA}} = 3$ following \citet{Huang2019} who explored the number of PCs necessary for an LSST Y10 analysis. The $\{Q_i\}$ are fast parameters, hence not included in the emulator training.

\subsubsection{Intrinsic alignment}\label{sssec:ia}

We model the intrinsic alignment using a redshift-dependent non-linear alignment (NLA) model \citep{Bridle2007}. In this model, the change in the angular power spectrum due to IA is modelled using a redshift dependent amplitude,
\begin{equation}
    A_{\text{IA}}(z) = -a_{\ia}\frac{C_1 \rho_{\text{cr}} \Omega_m}{G(z)}\bigg(\frac{1+z}{1+z_{0,\text{IA}}}\bigg)^{\eta_{\ia}},
\end{equation}
where, $C_1 \rho_{\text{cr}} = 0.0134$, $z_{0,\text{IA}} = 0.62$, $G(z)$ is the linear growth factor. There are only two free parameters in this model -- $a_{\ia}, \eta_{\ia}$ that parameterize the amplitude and the redshift dependence of the IA signal, respectively. For further details on our exact intrinsic alignment modeling, we refer to \citet{Krause2016, DESC_SRD, Krause2021}. 

For additional complexity of IA modeling we refer to \cite{Blazek2019} \cyan{pls cite more people}. IA parameters are slow parameters that are included in the emulator training. 
% We note that modeling the IA on smaller scales could require going beyond the simple tidal alignment model and include the impact of tidal torquing as well \citep{Blazek2019}. 


\subsubsection{Shear multiplicative bias}\label{sssec:shear_m}

We model possible biases in the shear inference through a multiplicative factor
\begin{equation}
    \gamma_{\text{measured}} = (1 + m)\times \gamma_{\text{true}}.
\end{equation}
Specifically, we add an extra parameter $m^i$ for each tomographic bin, which modifies the modeled observables as:
\begin{align}
    \xi^{ij}_{\pm} &\rightarrow (1 + m^i) (1 + m^j) \xi^{ij}_{\pm}, \\
    \gamma^{ij}_{t} &\rightarrow (1 + m^i) \gamma^{ij}_{t}.
\end{align}
The $m^i$ are fast parameters, hence not included in the emulator training.

\subsubsection{Galaxy bias}\label{sssec:gbias}
Following the DESC SRD we only include linear galaxy bias in our model. As we will see in section \ref{ssec:impact_studies}, this choice does not bias cosmological constraints given the DESC SRD scale cuts.
Linear galaxy bias changes the galaxy-galaxy lensing and the galaxy clustering part of the data vector as,
\begin{align}
    \gamma^{ij}_{t}(b^{j}_g) &= \bigg( \frac{b^{j}_g}{b^{j}_{g,\text{fid}}} \bigg) \times \gamma^{ij}_{t}(b^{j}_g = b^{j}_{g,\text{fid}}), \\
    w^i(b^{i}_g) &= \bigg(\frac{b^{i}_g}{b^{i}_{g,\text{fid}}}\bigg)^2 \times w^i (b^{i}_g = b^{i}_{g,\text{fid}}).
\end{align}
% Since the impact of linear galaxy bias is a simple multiplication on the data vector, we treat it as a fast parameter whose impact is not included in the emulator. While creating the training data for the emulator, we fix the linear galaxy bias to their fiducial value, $b_{g,\text{fid}}$. 
The fiducial value for the galaxy bias in the $i$-th redshift bin is set to $b_i = 1.05 / G(\bar{z}_i)$, where $G$ is the growth function and $\bar{z}_i$ is the mean redshift of the $i$-th redshift bin. The $b^{i}_g$ are fast parameters, hence not included in the emulator training.
%\cyan{This evolution is galaxy bias is consistent with what was founf by \citet{Nicola2020} with HSC data.}

\subsection{Angular binning and scale cuts}\label{ssec:scale_cuts}

We bin the data vectors in 20 logarithmically spaced angular bins, ranging from 1 arcminute to 400 arcminutes. To minimize the impact of baryonic physics and non-linear galaxy bias on cosmological results we adopt the DESC-SRD scale cuts with minor changes given that our 3x2 analysis is conducted in real space. The scale cuts for galaxy-galaxy lensing and galaxy clustering are obtained by applying the real space cut of $21~h^{-1}$ Mpc, approximately corresponding to the DESC-SRD cut of $k_{\text{max}} = 0.3~h$ Mpc$^{-1}$) to angular scales. For cosmic shear the DESC-SRD's $\ell_{\text{max}} = 3000$ limit is converted to real-space as $\theta_{\text{max}} = 2.756 (8.696)$ arcmin for $\xi_{+/-}$, so that $\ell_{\text{max}} \theta_{\text{min}}$ corresponds to the first zero of the Bessel function $J_{0/4}$. 

In section \ref{sec:small_scales}, we evaluate the science return and potential biases from imperfect modeling choices by extending the analysis to smaller scales.
